Escaping Saddle Points for Effective Generalization on Class-Imbalanced Data

Real-world datasets exhibit imbalances of varying types and degrees. Several techniques based on re-weighting and margin adjustment of loss are often used to enhance the performance of neural networks, particularly on minority classes. In this work, we analyze the class-imbalanced learning problem by examining the loss landscape of neural networks trained with re-weighting and margin-based techniques. Specifically, we examine the spectral density of Hessian of class-wise loss, through which we observe that the network weights converge to a saddle point in the loss landscapes of minority classes. Following this observation, we also find that optimization methods designed to escape from saddle points can be effectively used to improve generalization on minority classes. We further theoretically and empirically demonstrate that Sharpness-Aware Minimization (SAM), a recent technique that encourages convergence to a flat minima, can be effectively used to escape saddle points for minority classes. Using SAM results in a 6.2\% increase in accuracy on the minority classes over the state-of-the-art Vector Scaling Loss, leading to an overall average increase of 4\% across imbalanced datasets. The code is available at: https://github.com/val-iisc/Saddle-LongTail.

==> table.tex <==
\usepackage[numbers]{natbib}
\usepackage[final,nonatbib]{neurips_2022}

\usepackage[noend]{algpseudocode}
\usepackage[utf8]{inputenc} %
\usepackage[T1]{fontenc}    %
\usepackage{url}            %
\usepackage{booktabs}       %
\usepackage{amsfonts}       %
\usepackage{nicefrac}       %
\usepackage{microtype}      %
\usepackage{xcolor}   
\definecolor{darkpastelgreen}{rgb}{0.01, 0.75, 0.24}%
\usepackage[pagebackref=true,breaklinks=true,colorlinks,citecolor=darkpastelgreen,bookmarks=false]{hyperref}
\usepackage{soul}
\usepackage{multirow}
\usepackage{preamble}
\usepackage{bbm}
\def\sS{{\mathbb{S}}}
\def\sB{{\mathbb{B}}}
\usepackage{bbm}
\usepackage{preamble}
\usepackage{tikz}
\newcommand{\etal}{\textit{et al}.} 
\newcommand{\ie}{\textit{i}.\textit{e}. }
\newcommand{\eg}{\textit{e}.\textit{g}. }
\newcommand\Tstrut{\rule{0pt}{2.6ex}}         %
\newcommand\Bstrut{\rule[-0.9ex]{0pt}{0pt}}   %
\usepackage{adjustbox} %
\newcommand{\hrnote} [1]
{\textcolor{blue}{[HR: #1]}}
\usepackage{}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{wrapfig} %
\usepackage{multirow} %
\definecolor{mygray}{gray}{0.9} %
\usepackage[table]{colortbl}
\usepackage{algorithm}
\newcolumntype{?}{!{\vrule width 1pt}}

\begin{document}
\begin{table}
  \caption{Results on CIFAR-10 LT and CIFAR-100 LT with various methods that escape saddle points.}
  \label{tab:lpf_sgd}
  \centering
  \begin{adjustbox}{max width=\linewidth}
  \begin{tabular}{l|ll|ll}
    \toprule
    \multicolumn{1}{c}{}  & \multicolumn{2}{c}{CIFAR-10 LT}& \multicolumn{2}{c}{CIFAR-100 LT}\\
    
    \cmidrule(r){1-5}
     &Acc & Tail & Acc & Tail \\
    \midrule

    CE + DRW & 75.5 & 61.4 & 41.0 & 14.7 \Tstrut{}\\
    CE + DRW + PGD \cite{jin2017escape} & 77.2 & 65.0 & 42.2 & 17.0\\
    CE + DRW + LPF-SGD \cite{bisla2022low} & 78.5 & 67.2 & 42.9 & 15.8\\
    CE + DRW + SAM & 80.6 & 73.1  & 44.6 & 20.7
    \Bstrut{}\\

    
    \bottomrule
  \end{tabular}

  \end{adjustbox}
\end{table}

\begin{table}
  \caption{Results on CIFAR-10 LT and CIFAR-100 LT with $\beta$=100. SAM with re-weighting is able to avoid the regions of negative curvature, leading to major gain in performance on the mid and tail classes with CE, LDAM and VS.}
  \label{tab:cifar_lt}
  \centering
  \begin{adjustbox}{max width=\linewidth}
  \begin{tabular}{l|ll | ll}
    \toprule
    \multicolumn{1}{c}{}  & \multicolumn{2}{c}{CIFAR-10 LT}& \multicolumn{2}{c}{CIFAR-100 LT}\\
    
    \cmidrule(r){1-5}
     &Acc  & Tail & Acc  & Tail  \\
    \midrule
    CE & 71.7\[_{\pm 0.1}\]  & 52.3\[_{\pm 3.7}\] & 38.5\[_{\pm 0.5}\] & 8.2\[_{\pm 1.0}\]\\
    \rowcolor{mygray} CE + SAM & 73.1\[_{\pm 0.3}\]   & 51.7\[_{\pm 1.0}\] & 39.6\[_{\pm 0.6}\] & 8.0\[_{\pm 0.6}\]  \Bstrut{}\\
\hline
    CE + DRW \cite{cao2019learning} & 75.5\[_{\pm 0.2}\] & 61.4\[_{\pm 0.9}\] & 41.0\[_{\pm 0.6}\]  & 14.7\[_{\pm 0.9}\] \Tstrut{}\\
    \rowcolor{mygray}
    \rowcolor{mygray} CE + DRW + SAM & 80.6\[_{\pm 0.4}\] & 73.1 \[_{\pm 0.9}\] & 44.6\[_{\pm 0.4}\] & 20.7\[_{\pm 0.6}\]  \Bstrut{}\\
    \hline
    LDAM + DRW \cite{cao2019learning} & 77.5\[_{\pm 0.5}\]  & 66.4\[_{\pm 0.2}\] & 42.7\[_{\pm 0.3}\] & 19.4\[_{\pm 0.9}\] \Tstrut{}\\
    \rowcolor{mygray} LDAM + DRW + SAM & 81.9\[_{\pm 0.4}\] & 76.4 \[_{\pm 1.1}\] & 45.4\[_{\pm 0.1}\] & 20.8 $_{\pm 0.3}$  \Bstrut{}\\
    \hline
    VS \cite{kini2021label} & 78.6$_{\pm 0.3}$  & 70.3$_{\pm 0.5}$ & 41.7$_{\pm 0.5}$ & 26.8$_{\pm 1.0}$  \Tstrut{}\\
    \rowcolor{mygray} VS + SAM & 82.4$_{\pm 0.4}$ & 78.0$_{\pm 01.2}$ & 46.6$_{\pm 0.4}$ & 31.7$_{\pm 0.1}$ \Bstrut{}\\

    
    \bottomrule
  \end{tabular}

  \end{adjustbox}
\end{table}

    


    



\end{document}

